Variance-Reduced Conservative Policy Iteration

We study the sample complexity of reducing reinforcement learning to a sequence of empirical risk minimization problems over the policy space. Such reductions-based algorithms exhibit local convergence in the function space, as opposed to the parameter space for policy gradient algorithms, and thus are unaffected by the possibly non-linear or discontinuous parameterization of the policy class. We propose a variance-reduced variant of Conservative Policy Iteration that improves the sample complexity of producing a $\varepsilon$-functional local optimum from $O(\varepsilon^{-4})$ to $O(\varepsilon^{-3})$. Under state-coverage and policy-completeness assumptions, the algorithm enjoys $\varepsilon$-global optimality after sampling $O(\varepsilon^{-2})$ times, improving upon the previously established $O(\varepsilon^{-3})$ sample requirement.

==> format/neurips-defs.tex <==
%%%%%% GENERIC FORMATTING %%%%%%
%\numberwithin{equation}{section}

%%%%%%%%%%%%% SPECIFIC UTILS %%%%%%%%%%%%%%%

\newcommand{\policynorm}[1]{\| #1 \|}
\def\ic{\lambda}
% Editing macros
\newcommand{\ks}[1]{{\color{red}[KS: #1]}}
\newcommand{\na}[1]{{\color{purple}[NA: #1]}}
\newcommand{\bb}[1]{{\color{green}[BB: #1]}}

%%%%%%%%%%%%% MATH UTILS %%%%%%%%%%%%%%%

\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\def\reals{{\mathbb R}}
\newcommand{\eps}{\varepsilon}
\newcommand{\defeq}{\triangleq}
\def\regret{\ensuremath{\mbox{Regret}}}

\def\grad{\nabla}
\def\hess{\nabla^2}
\def\hessinv{\nabla^{-2}}
\def\hestinv{\tilde{\nabla}^{-2}}
\def\hest{\tilde{\nabla}^{2}}

% operators
\def\norm#1{\mathopen\| #1 \mathclose\|}
\newcommand{\innerprod}[2]{\langle #1, #2 \rangle}
\newcommand{\matnorm}[2]{\| #1 \|_{#2}}
\newcommand{\invmatnorm}[2]{\| #1 \|_{#2^{-1}}}
\newcommand{\abs}[1]{\left|#1\right|}

% brackets
\newcommand{\braces}[1]{\left\{#1\right\}}
\newcommand{\pa}[1]{\left(#1\right)}
\newcommand{\ang}[1]{\left<#1\right>}
\newcommand{\bra}[1]{\left[#1\right]}

\newcommand\mycases[4] {{
\left\{
\begin{array}{ll}
    {#1} & {#2} \\\\
    {#3} & {#4}
\end{array}
\right. }}





%%%%%%%%%%%%% THEOREMS AND REP THEOREMS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{construction}[theorem]{Construction}
\newtheorem{algorithm1}[theorem]{Algorithm}
\newtheorem{protocol}[theorem]{Protocol}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{example}[theorem]{Example}

\newcommand{\newreptheorem}[2]{%
\newenvironment{rep#1}[1]{%
 \def\rep@title{#2 \ref{##1}}%
 \begin{rep@theorem}}%
 {\end{rep@theorem}}}
\newreptheorem{theorem}{Theorem}
\newreptheorem{lemma}{Lemma}
\newreptheorem{proposition}{Proposition}
\newreptheorem{claim}{Claim}
\newreptheorem{corollary}{Corollary}
\newreptheorem{mainlemma}{Main Lemma}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% prettyref

\usepackage{prettyref}
\newcommand{\pref}[1]{\prettyref{#1}}
\newcommand{\pfref}[1]{Proof of \prettyref{#1}}
\newcommand{\savehyperref}[2]{\texorpdfstring{\hyperref[#1]{#2}}{#2}}
\newrefformat{eq}{\savehyperref{#1}{\textup{(\ref*{#1})}}}
\newrefformat{eqn}{\savehyperref{#1}{Equation~\ref*{#1}}}
\newrefformat{lem}{\savehyperref{#1}{Lemma~\ref*{#1}}}
\newrefformat{def}{\savehyperref{#1}{Definition~\ref*{#1}}}
\newrefformat{thm}{\savehyperref{#1}{Theorem~\ref*{#1}}}
\newrefformat{cor}{\savehyperref{#1}{Corollary~\ref*{#1}}}
\newrefformat{sec}{\savehyperref{#1}{Section~\ref*{#1}}}
\newrefformat{app}{\savehyperref{#1}{Appendix~\ref*{#1}}}
\newrefformat{ass}{\savehyperref{#1}{Assumption~\ref*{#1}}}
\newrefformat{ex}{\savehyperref{#1}{Example~\ref*{#1}}}
\newrefformat{fig}{\savehyperref{#1}{Figure~\ref*{#1}}}
\newrefformat{alg}{\savehyperref{#1}{Algorithm~\ref*{#1}}}
\newrefformat{rem}{\savehyperref{#1}{Remark~\ref*{#1}}}
\newrefformat{conj}{\savehyperref{#1}{Conjecture~\ref*{#1}}}
\newrefformat{prop}{\savehyperref{#1}{Proposition~\ref*{#1}}}
\newrefformat{proto}{\savehyperref{#1}{Protocol~\ref*{#1}}}
\newrefformat{prob}{\savehyperref{#1}{Problem~\ref*{#1}}}
\newrefformat{claim}{\savehyperref{#1}{Claim~\ref*{#1}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%% ALL LETTERS %%%%%%%

\def\A{{\mathcal A}}
\def\B{{\mathcal B}}
\def\C{{\mathcal C}}
\def\D{{\mathcal D}}
\def\E{{\mathcal E}}
\def\F{{\mathcal F}}
\def\G{{\mathcal G}}
\def\H{{\mathcal H}}
\def\I{{\mathcal I}}
\def\J{{\mathcal J}}
\def\K{{\mathcal K}}
\def\L{{\mathcal L}}
\def\M{{\mathcal M}}
\def\N{{\mathcal N}}
\def\O{{\mathcal O}}
\def\P{{\mathcal P}}
\def\Q{{\mathcal Q}}
\def\R{{\mathcal R}}
\def\S{{\mathcal S}}
\def\T{{\mathcal T}}
\def\U{{\mathcal U}}
\def\V{{\mathcal V}}
\def\W{{\mathcal W}}
\def\X{{\mathcal X}}
\def\Y{{\mathcal Y}}
\def\Z{{\mathcal Z}}

% \def\bA{\mathbf{A}}
% \def\bB{\mathbf{B}}
% \def\bC{\mathbf{C}}
% \def\bD{\mathbf{D}}
% \def\bE{\mathbf{E}}
% \def\bF{\mathbf{F}}
% \def\bG{\mathbf{G}}
% \def\bH{\mathbf{H}}
% \def\bI{\mathbf{I}}
% \def\bJ{\mathbf{J}}
% \def\bK{\mathbf{K}}
% \def\bL{\mathbf{L}}
% \def\bM{\mathbf{M}}
% \def\bN{\mathbf{N}}
% \def\bO{\mathbf{O}}
% \def\bP{\mathbf{P}}
% \def\bQ{\mathbf{Q}}
% \def\bR{\mathbf{R}}
% \def\bS{\mathbf{S}}
% \def\bT{\mathbf{T}}
% \def\bU{\mathbf{U}}
% \def\bV{\mathbf{V}}
% \def\bW{\mathbf{W}}
% \def\bX{\mathbf{X}}
% \def\bY{\mathbf{Y}}
% \def\bZ{\mathbf{Z}}


% \def\ba{\mathbf{a}}
% \def\bb{\mathbf{b}}
% \def\bc{\mathbf{c}}
% \def\bd{\mathbf{d}}
% \def\be{\mathbf{e}}
% \def\bf{\mathbf{f}}
% \def\bg{\mathbf{g}}
% \def\bh{\mathbf{h}}
% \def\bi{\mathbf{i}}
% \def\bj{\mathbf{j}}
% \def\bk{\mathbf{k}}
% \def\bl{\mathbf{l}}
% \def\bm{\mathbf{m}}
% \def\bn{\mathbf{n}}
% \def\bo{\mathbf{o}}
% \def\bp{\mathbf{p}}
% \def\bq{\mathbf{q}}
% \def\br{\mathbf{r}}
% \def\bs{\mathbf{s}}
% \def\bt{\mathbf{t}}
% \def\bu{\mathbf{u}}
% \def\bv{\mathbf{v}}
% \def\bw{\mathbf{w}}
% \def\bx{\mathbf{x}}
% \def\by{\mathbf{y}}
% \def\bz{\mathbf{z}}

\def\bbA{{\mathbb A}}
\def\bbB{{\mathbb B}}
\def\bbC{{\mathbb C}}
\def\bbD{{\mathbb D}}
\def\bbE{{\mathbb E}}
\def\bbF{{\mathbb F}}
\def\bbG{{\mathbb G}}
\def\bbH{{\mathbb H}}
\def\bbI{{\mathbb I}}
\def\bbJ{{\mathbb J}}
\def\bbK{{\mathbb K}}
\def\bbL{{\mathbb L}}
\def\bbM{{\mathbb M}}
\def\bbN{{\mathbb N}}
\def\bbO{{\mathbb O}}
\def\bbP{{\mathbb P}}
\def\bbQ{{\mathbb Q}}
\def\bbR{{\mathbb R}}
\def\bbS{{\mathbb S}}
\def\bbT{{\mathbb T}}
\def\bbU{{\mathbb U}}
\def\bbV{{\mathbb V}}
\def\bbW{{\mathbb W}}
\def\bbX{{\mathbb X}}
\def\bbY{{\mathbb Y}}
\def\bbZ{{\mathbb Z}}


%\DeclareMathOperator{\sign}{sign}


==> main/__latexindent_temp.tex <==
\section{Analysis}
\subsection{Proof of the main result}
\begin{proof}[Proof of Theorem~\ref{thm:mainlocal}]
    Let us first observe that value function $V^\pi_\mu$ is a smooth over the space of policies. The following statement holds independently of how the policy class itself may be parameterized.
    
    \begin{lemma}
      \label{lem:smooth}
      For any start-state distribution $\mu$, $V^\pi_\mu$ is $\frac{2\gamma}{(1-\gamma)^3}$-smooth in the $\|\cdot\|_{\infty,1}$ norm.
    \end{lemma}
    
    We invoke smoothness of $V^\pi_\mu$, as Lemma~\ref{lem:smooth} certifies, to observe that since successive iterates are close in the $\|\cdot\|_{\infty,1}$ norm, we have 
    \begin{align*}
      V^{\pi_{t+1}}_\mu &= V^{\pi_{t}+\eta(\pi'_t-\pi_t)}_\mu\\
      &\geq  V^{\pi_t}_\mu + \eta \langle \nabla V^{\pi_t}_\mu, \pi'_t-\pi_t\rangle - \frac{\gamma \eta^2}{(1-\gamma)^3} \|\pi'_{t}-\pi_t  \|_{\infty,1}^2.
    \end{align*}
    
    Next, we wish to use the fact to fact that $\pi'_t$ was chosen by a ERM oracle, and therefore approximately maximizes the inner product with the gradient of the value function. To do this, we first relate the ERM objective (as in Algorithm~\ref{alg:cpi}) to the said gradient.

    \begin{theorem}
        \label{thm:varmain}
        For Algorithm~\ref{alg:cpi}, for all times $t\leq T$, define $d_t\in \reals^{S\times A}$ such that for any policy $\pi$, the ERM loss for $\pi$ on $D_t$ may be expressed as 
        $$ \langle d_t,\pi\rangle = \sum_{i=1}^{3t} \widehat{l}_i^\top \pi(s_i). $$ 
        Then for any $\eta < 1/4$ and $a = 4\eta$, for any $\varepsilon, \delta$, with probability at least $1 - \delta$, we have that for all policies $\pi \in \Pi$ and time $t \leq T$
        \[|\innerprod{d_t - \nabla V^{\pi_t}_\mu}{\pi}| \leq 2(1-4\eta)^t + \sqrt{32\eta\ln(2 |\Pi_{\varepsilon}|T/\delta)} + 9/4\varepsilon.\]
    \end{theorem}

    Note that the above inequality (in Theorem~\ref{thm:varmain}) also holds for policies, such as iterates $\pi_t$ of Algorithm~\ref{alg:cpi}, in the convex hull of $\Pi$ since $f(\pi)=\max\{\innerprod{d_t - \nabla V^{\pi_t}_\mu}{\pi}, -\innerprod{d_t - \nabla V^{\pi_t}_\mu}{\pi}\}$ is convex in $\pi$, thereby implying that that extreme values are realized at the boundary, i.e. $\Pi$.
    
    An $\varepsilon$-tolerant Empirical Risk Minimization Oracle, by its definition, guarantees for any $t$
    \begin{align*}
      \max_{\pi^*\in \Pi} \langle \nabla V^{\pi_t}_\mu, \pi^* - \pi'_t \rangle &\leq \max_{\pi^*\in \Pi} \langle d_t, \pi^* - \pi'_t \rangle + 2\max_{\pi\in \Pi} |\langle d_t -\nabla V^{\pi_t}_\mu , \pi \rangle | \\
      &= \max_{\pi^*\in \Pi}\sum_{i=0}^{3t} \widehat{l}_i^\top (\pi^*(s_i)-\pi'_t(s_i)) + 2\max_{\pi\in \Pi} |\langle d_t -\nabla V^{\pi_t}_\mu , \pi\rangle | \\
      &\leq\varepsilon + 2\max_{\pi\in \Pi} |\langle d_t -\nabla V^{\pi_t}_\mu , \pi\rangle | 
    \end{align*}
    
    Using the bound indicated in Theorem~\ref{thm:varmain}, with probability $1-\delta$, for all $t$, the inequality concerning successive iterates may thus be written as 
    \begin{align*}
      &\max_{\pi^*\in \Pi}\langle \nabla V^{\pi_t}_\mu, \pi^*_t-\pi_t\rangle \\
      =& \max_{\pi^*\in \Pi}\langle \nabla V^{\pi_t}_\mu, \pi^*_t-\pi'_t\rangle +\langle \nabla V^{\pi_t}_\mu, \pi'_t-\pi_t\rangle\\
    \leq& \varepsilon + 2\max_{\pi\in \Pi} |\langle d_t -\nabla V^{\pi_t}_\mu , \pi\rangle | + \langle \nabla V^{\pi_t}_\mu, \pi'_t-\pi_t\rangle \\
      \leq &  4(1-4\eta)^t + 16\sqrt{\eta\log\frac{2 |\Pi_{\varepsilon}|T}{\delta}} + 6\varepsilon + \frac{V^{\pi_{t+1}}_\mu - V^{\pi_t}_\mu}{\eta} + \frac{4\gamma \eta}{(1-\gamma)^3}.
    \end{align*}
    where the last inequality uses that for any policy $\pi$, $\|\pi\|_{\infty,1}=1$, and therefore, $\|\pi'_t-\pi_t\|_{\infty,1}\leq 2$.
    
    Since value functions are always bounded by $\frac{1}{1-\gamma}$, we telescope the inequality and average over iterations to observe that with probability $1-\delta$ 
    \begin{align}
      \label{eq:avggua}
      \frac{1}{T}\sum_{t=1}^T\max_{\pi^*\in \Pi}\langle \nabla V^{\pi_t}_\mu, \pi^*_t-\pi_t\rangle &\leq  4(1-4\eta)^t + 16\sqrt{\eta\log\frac{2 |\Pi_{\varepsilon}|T}{\delta}} + 6\varepsilon + \frac{1}{\eta (1-\gamma)T} + \frac{4\gamma \eta}{(1-\gamma)^3} .
    \end{align}
  
    Now, finally, we move from an average to a guarantee on a specific iterate. From, we have that 
    \begin{align*}
      &\left\lvert  \widehat{A}_t - \max_{\pi^*\in\Pi}\langle \nabla V^{\pi_t}_\mu, \pi^*-\pi_t\rangle \right\rvert \\
      =& \left\lvert  \langle d_t, \pi'_t-\pi_t\rangle - \max_{\pi^*\in\Pi}\langle \nabla V^{\pi_t}_\mu, \pi^*-\pi_t\rangle \right\rvert\\
      \leq& \max \{  \langle d_t, \pi'_t-\pi^*_t\rangle,  \max_{\pi^*\in \Pi}\langle \nabla V^{\pi_t}_\mu, \pi^*_t-\pi'_t\rangle \} + 2\max_{\pi\in \Pi} |\langle d_t -\nabla V^{\pi_t}_\mu , \pi \rangle |  \\
      \leq& \varepsilon +  2\max_{\pi\in \Pi} |\langle d_t -\nabla V^{\pi_t}_\mu , \pi \rangle | 
    \end{align*}
    
    Let $\bar{t}=\argmin_t \widehat{A}_t$ and $t'= \argmin_t \max_{\pi^*} \langle \nabla V^{\pi_t}_\mu, \pi^* - \pi_t\rangle$. Since $\bar{t}$ and $t'$ are random, we take a union bound on the preceding claim for all $\widehat{A}_t$. Then it follows with probability $1-\delta$, by definition of $t'$ and $\bar{t}$, that
    \begin{align*}
      &\max_{\pi^*\in \Pi}\langle \nabla V^{\pi_{\bar{t}}}_\mu, \pi^*-\pi_{\bar{t}}\rangle \\
      \leq & \widehat{A}_{\bar{t}}+\varepsilon +  2\max_{\pi\in \Pi} |\langle d_t -\nabla V^{\pi_t}_\mu , \pi \rangle |  \\
      \leq & \widehat{A}_{t'} +\varepsilon +  2\max_{\pi\in \Pi} |\langle d_t -\nabla V^{\pi_t}_\mu , \pi \rangle | \\
      \leq & \min_t\max_{\pi^*\in \Pi} \langle \nabla V^{\pi_t}_\mu, \pi^*-\pi_t\rangle+2\varepsilon +  4\max_{\pi\in \Pi} |\langle d_t -\nabla V^{\pi_t}_\mu , \pi \rangle | \\
      \leq & \frac{1}{T}\sum_{t=1}^T\max_{\pi^*\in \Pi} \langle \nabla V^{\pi_t}_\mu, \pi^*-\pi_t\rangle +2\varepsilon +  4\max_{\pi\in \Pi} |\langle d_t -\nabla V^{\pi_t}_\mu , \pi \rangle | \\
      \leq& 12(1-4\eta)^t + 48\sqrt{\eta\log\frac{2 |\Pi_{\varepsilon}|T}{\delta}} + 17\varepsilon + \frac{1}{\eta (1-\gamma)T} + \frac{4\gamma \eta}{(1-\gamma)^3}
    \end{align*}
    where the last inequality follows from the average iterate guarantee in Equation~\ref{eq:avggua}.
\end{proof}

\subsection{Proof of faster global convergence}
\begin{proof}[Proof of Theorem~\ref{thm:fast}]
        Let us first observe that value function $V^\pi_\mu$ is a smooth over the space of policies. The following statement holds independently of how the policy class itself may be parameterized.
        
        \begin{lemma}
          \label{lem:smooth}
          For any start-state distribution $\mu$, $V^\pi_\mu$ is $\frac{2\gamma}{(1-\gamma)^3}$-smooth in the $\|\cdot\|_{\infty,1}$ norm.
        \end{lemma}
        
        We invoke smoothness of $V^\pi_\mu$, as Lemma~\ref{lem:smooth} certifies, to observe that since successive iterates are close in the $\|\cdot\|_{\infty,1}$ norm, we have 
        \begin{align*}
          V^{\pi_{t+1}}_\mu &= V^{\pi_{t}+\eta(\pi'_t-\pi_t)}_\mu\\
          &\geq  V^{\pi_t}_\mu + \eta \langle \nabla V^{\pi_t}_\mu, \pi'_t-\pi_t\rangle - \frac{\gamma \eta^2}{(1-\gamma)^3} \|\pi'_{t}-\pi_t  \|_{\infty,1}^2.
        \end{align*}
        
        Next, we wish to use the fact to fact that $\pi'_t$ was chosen by a ERM oracle, and therefore approximately maximizes the inner product with the gradient of the value function. To do this, we first relate the ERM objective (as in Algorithm~\ref{alg:cpi}) to the said gradient.
    
        \begin{theorem}
            \label{thm:varmain}
            For Algorithm~\ref{alg:cpi}, for all times $t\leq T$, define $d_t\in \reals^{S\times A}$ such that for any policy $\pi$, the ERM loss for $\pi$ on $D_t$ may be expressed as 
            $$ \langle d_t,\pi\rangle = \sum_{i=1}^{3t} \widehat{l}_i^\top \pi(s_i). $$ 
            Then for any $\eta < 1/4$ and $a = 4\eta$, for any $\varepsilon, \delta$, with probability at least $1 - \delta$, we have that for all policies $\pi \in \Pi$ and time $t \leq T$
            \[|\innerprod{d_t - \nabla V^{\pi_t}_\mu}{\pi}| \leq 2(1-4\eta)^t + \sqrt{32\eta\ln(2 |\Pi_{\varepsilon}|T/\delta)} + 9/4\varepsilon.\]
        \end{theorem}
    
        Note that the above inequality (in Theorem~\ref{thm:varmain}) also holds for policies, such as iterates $\pi_t$ of Algorithm~\ref{alg:cpi}, in the convex hull of $\Pi$ since $f(\pi)=\max\{\innerprod{d_t - \nabla V^{\pi_t}_\mu}{\pi}, -\innerprod{d_t - \nabla V^{\pi_t}_\mu}{\pi}\}$ is convex in $\pi$, thereby implying that that extreme values are realized at the boundary, i.e. $\Pi$.
        
        An $\varepsilon$-tolerant Empirical Risk Minimization Oracle, by its definition, guarantees for any $t$
        \begin{align*}
          \max_{\pi^*\in \Pi} \langle \nabla V^{\pi_t}_\mu, \pi^* - \pi'_t \rangle &\leq \max_{\pi^*\in \Pi} \langle d_t, \pi^* - \pi'_t \rangle + 2\max_{\pi\in \Pi} |\langle d_t -\nabla V^{\pi_t}_\mu , \pi \rangle | \\
          &= \max_{\pi^*\in \Pi}\sum_{i=0}^{3t} \widehat{l}_i^\top (\pi^*(s_i)-\pi'_t(s_i)) + 2\max_{\pi\in \Pi} |\langle d_t -\nabla V^{\pi_t}_\mu , \pi\rangle | \\
          &\leq\varepsilon + 2\max_{\pi\in \Pi} |\langle d_t -\nabla V^{\pi_t}_\mu , \pi\rangle | 
        \end{align*}
        
        Using the bound indicated in Theorem~\ref{thm:varmain}, with probability $1-\delta$, for all $t$, the inequality concerning successive iterates may thus be written as 
        \begin{align*}
          &\max_{\pi^*\in \Pi}\langle \nabla V^{\pi_t}_\mu, \pi^*_t-\pi_t\rangle \\
          =& \max_{\pi^*\in \Pi}\langle \nabla V^{\pi_t}_\mu, \pi^*_t-\pi'_t\rangle +\langle \nabla V^{\pi_t}_\mu, \pi'_t-\pi_t\rangle\\
        \leq& \varepsilon + 2\max_{\pi\in \Pi} |\langle d_t -\nabla V^{\pi_t}_\mu , \pi\rangle | + \langle \nabla V^{\pi_t}_\mu, \pi'_t-\pi_t\rangle \\
          \leq &  4(1-4\eta)^t + 16\sqrt{\eta\log\frac{2 |\Pi_{\varepsilon}|T}{\delta}} + 6\varepsilon + \frac{V^{\pi_{t+1}}_\mu - V^{\pi_t}_\mu}{\eta} + \frac{4\gamma \eta}{(1-\gamma)^3}.
        \end{align*}
        where the last inequality uses that for any policy $\pi$, $\|\pi\|_{\infty,1}=1$, and therefore, $\|\pi'_t-\pi_t\|_{\infty,1}\leq 2$.
        
        Since value functions are always bounded by $\frac{1}{1-\gamma}$, we telescope the inequality and average over iterations to observe that with probability $1-\delta$ 
        \begin{align}
          \label{eq:avggua}
          \frac{1}{T}\sum_{t=1}^T\max_{\pi^*\in \Pi}\langle \nabla V^{\pi_t}_\mu, \pi^*_t-\pi_t\rangle &\leq  4(1-4\eta)^t + 16\sqrt{\eta\log\frac{2 |\Pi_{\varepsilon}|T}{\delta}} + 6\varepsilon + \frac{1}{\eta (1-\gamma)T} + \frac{4\gamma \eta}{(1-\gamma)^3} .
        \end{align}
      
        Now, finally, we move from an average to a guarantee on a specific iterate. From, we have that 
        \begin{align*}
          &\left\lvert  \widehat{A}_t - \max_{\pi^*\in\Pi}\langle \nabla V^{\pi_t}_\mu, \pi^*-\pi_t\rangle \right\rvert \\
          =& \left\lvert  \langle d_t, \pi'_t-\pi_t\rangle - \max_{\pi^*\in\Pi}\langle \nabla V^{\pi_t}_\mu, \pi^*-\pi_t\rangle \right\rvert\\
          \leq& \max \{  \langle d_t, \pi'_t-\pi^*_t\rangle,  \max_{\pi^*\in \Pi}\langle \nabla V^{\pi_t}_\mu, \pi^*_t-\pi'_t\rangle \} + 2\max_{\pi\in \Pi} |\langle d_t -\nabla V^{\pi_t}_\mu , \pi \rangle |  \\
          \leq& \varepsilon +  2\max_{\pi\in \Pi} |\langle d_t -\nabla V^{\pi_t}_\mu , \pi \rangle | 
        \end{align*}
        
        Let $\bar{t}=\argmin_t \widehat{A}_t$ and $t'= \argmin_t \max_{\pi^*} \langle \nabla V^{\pi_t}_\mu, \pi^* - \pi_t\rangle$. Since $\bar{t}$ and $t'$ are random, we take a union bound on the preceding claim for all $\widehat{A}_t$. Then it follows with probability $1-\delta$, by definition of $t'$ and $\bar{t}$, that
        \begin{align*}
          &\max_{\pi^*\in \Pi}\langle \nabla V^{\pi_{\bar{t}}}_\mu, \pi^*-\pi_{\bar{t}}\rangle \\
          \leq & \widehat{A}_{\bar{t}}+\varepsilon +  2\max_{\pi\in \Pi} |\langle d_t -\nabla V^{\pi_t}_\mu , \pi \rangle |  \\
          \leq & \widehat{A}_{t'} +\varepsilon +  2\max_{\pi\in \Pi} |\langle d_t -\nabla V^{\pi_t}_\mu , \pi \rangle | \\
          \leq & \min_t\max_{\pi^*\in \Pi} \langle \nabla V^{\pi_t}_\mu, \pi^*-\pi_t\rangle+2\varepsilon +  4\max_{\pi\in \Pi} |\langle d_t -\nabla V^{\pi_t}_\mu , \pi \rangle | \\
          \leq & \frac{1}{T}\sum_{t=1}^T\max_{\pi^*\in \Pi} \langle \nabla V^{\pi_t}_\mu, \pi^*-\pi_t\rangle +2\varepsilon +  4\max_{\pi\in \Pi} |\langle d_t -\nabla V^{\pi_t}_\mu , \pi \rangle | \\
          \leq& 12(1-4\eta)^t + 48\sqrt{\eta\log\frac{2 |\Pi_{\varepsilon}|T}{\delta}} + 17\varepsilon + \frac{1}{\eta (1-\gamma)T} + \frac{4\gamma \eta}{(1-\gamma)^3}
        \end{align*}
        where the last inequality follows from the average iterate guarantee in Equation~\ref{eq:avggua}.
        \end{proof}



==> main/a-missing-details-neurips.tex <==
% \section{Missing Details from the main paper}

% % In this section we collect some simple artifacts from the main paper which we could not include in the main paper due to space constraints.

% % \paragraph{Example highlighting not all parameter space local optimal are functional local optima}



% % \paragraph{Lemma showing gradient domination property under policy class coverage}

% % The following lemma shows that the value function is approximately gradient dominated when every policy in the policy class has sufficient coverage under Definition \ref{def:disma2}.



% \paragraph{Sampling Algorithms}

% In this section we present our algorithms Q-Sampler(Algorithm \ref{alg:qsamp}) and H-Sampler(Algorithm \ref{alg:hsamp}). 






==> main/ignore.tex <==
\section{Old Stuff}
\begin{proof}
The first part of the theorem follows immediately via the definition of $d_t$ and the definition of the datasets $D_t$ in Algorithm \ref{alg:cpi}. We now proceed with the bound on the deviation. Remember that $d_t$ is defined in a recursive fashion by satisfying the following for any $\pi \in \B_{\infty,1}$,

\begin{align*} \langle d_t, \pi\rangle \defeq & (1-a) \langle d_{t-1}, \pi\rangle + a \cdot  \frac{\widehat{Q}_t^\top \pi (s_t)}{1-\gamma} \\&+ (1-a) \left(\frac{\gamma}{(1-\gamma)^2} \left( (\widehat{H}_t(\pi_t(s''_t)-\pi_{t-1}(s''_t)))^\top \pi(s'_t) +(\widehat{H}_t(\pi_t(s'_t)-\pi_{t-1}(s'_t)))^\top \pi(s''_t)  \right) \right).
    \end{align*}
For brevity in the proof we define the following random functions defined over all $\pi \in \B_{\infty, 1}$ and for all $t$
\[\psi_t(\pi) \defeq \frac{\widehat{Q}_t^\top \pi (s_t)}{1-\gamma}\]
\[\zeta_t(\pi) \defeq \frac{\gamma}{(1-\gamma)^2} \left( (\widehat{H}_t(\pi_t(s''_t)-\pi_{t-1}(s''_t)))^\top \pi(s'_t) +(\widehat{H}_t(\pi_t(s'_t)-\pi_{t-1}(s'_t)))^\top \pi(s''_t)  \right) \]
Therefore by definition we have that for all $\pi \in \B_{\infty, 1}$ and for all $t$,
\[\innerprod{d_t}{\pi} = (1-a)\innerprod{d_{t-1}}{\pi} + a \psi_t(\pi) + (1-a) \zeta_t(\pi).\]

Before moving onto the proof we will provide some simple upper bounds on the random variables $\psi_t(\pi), \zeta_t(\pi)$ for any $\pi \in \B_{\infty, 1}$. Using Claim \ref{lem:qsamp} we get that for any $t \leq T, \pi \in \B_{\infty, 1}$,
\begin{equation}
\label{eq:temppsi}
   |\psi_t(\pi)| \leq \frac{\|\hat{Q}_t\|_1 \|\pi(s_t)\|_{\infty}}{1-\gamma} \leq \frac{|A| \log(1/\varepsilon_Q (1 - \gamma))}{(1-\gamma)^2}.
\end{equation}
Further using Claim \ref{lem:hsamp} we get that for any $t \leq T, \pi \in \B_{\infty, 1}$, 
\begin{align}
   |\zeta_t(\pi)| &\leq \frac{\gamma}{(1-\gamma)^2}\left(\sum_{a,a' \in A \times A} |H(a,a')|\right)\|\pi(s_t')\|_{\infty}\left(\|\pi_t(s_t') - \pi_{t-1}(s_t')\|_{\infty} + \|\pi_t(s_t'') - \pi_{t-1}(s_t'')\|_{\infty} \right) \nonumber\\
   &\leq \frac{2 |A|^2\gamma \log(1/\varepsilon_H(1-\gamma))}{(1-\gamma)^3}\|\pi_t - \pi_{t-1}\|_{\infty, 1}.  \label{eq:tempzeta}
\end{align}
We now move on to the main proof. The idea will be to show the required statement for every policy $\pi \in \Pi_{\varepsilon}$ and then extend to the full set $\Pi$ via the covering property. To this end, fix a policy $\pi \in \Pi_{\varepsilon}$ and consider the following derivations. We will first show that $\innerprod{d_t}{\pi}$ concentrates to its expectation. 
Let $\bbE_{t}$ represent expectation fixing all the randomness upto and including time $t$. Next consider the definitions of the following sequences for every $t \geq 0$, 
\[\epsilon_t \defeq d_t - \bbE[d_t] \qquad y_t \defeq \frac{\innerprod{\epsilon_t}{\pi}}{(1-a)^t}.\]
We next show that the sequence $\{y_t\}$ is a martingale sequence over time $t$. To see this consider the following derivation, 
\begin{align*}
  \bbE_{t-1}[y_t] &= \frac{\bbE_{t-1}[\innerprod{\epsilon_t}{\pi}]}{(1-a)^t} =\frac{\bbE_{t-1}[\innerprod{(d_t - \bbE[d_{t}])}{\pi}]}{(1-a)^t} \\
   &= \frac{1}{(1-a)^t} \left( (1-a) \bbE_{t-1}[\innerprod{(d_{t-1} - \bbE[d_{t-1}])}{\pi}] + a \left(\bbE_{t-1}[\psi_t(\pi)] - \bbE[\psi_t(\pi)] \right) \right.\\
   & \left. \qquad \qquad + (1-a) \left( \bbE_{t-1}[\zeta_t(\pi)] - \bbE[\zeta_t(\pi)] \right) \right) \\
  &= \frac{(1-a)\innerprod{\epsilon_{t-1}}{\pi}}{(1-a)^t} = y_{t-1}  
\end{align*}
We now wish to use Azuma's inequality to show concentration for the martingale sequence. 
% Furthermore, note that for any policies $\pi, \pi'$ Lemma \ref{lem:grad} implies that $\innerprod{\nabla V_{\mu}^{\pi}}{\pi'} \leq \frac{1}{(1-\gamma)^2}$. 
Using the above derivations we can now bound the differences of the martingale sequences as follows which holds for all $t$ with probability $1$, 
\begin{align*}
    x_t \defeq |y_t - y_{t-1}| &=  \frac{|\epsilon_t - (1-a)\epsilon_{t-1}|}{(1-a)^t}  \\
    &= \frac{|a(\psi_t - \bbE[\psi_t(\pi)])| + |(1-a)(\zeta_t - \bbE[\zeta_t(\pi)])|}{(1-a)^t}\\
    &\leq  \frac{a \cdot\frac{2|A| \log(1/\varepsilon_Q (1 - \gamma))}{(1-\gamma)^2} + (1-a)\cdot\frac{4 |A|^2\gamma \log(1/\varepsilon_H(1-\gamma))}{(1-\gamma)^3}\|\pi_t - \pi_{t-1}\|_{\infty, 1} }{(1-a)^t} \\ 
    &\leq  \frac{a \cdot\frac{2|A| \log(1/\varepsilon_Q (1 - \gamma))}{(1-\gamma)^2} + (1-a)\eta\cdot\frac{4 |A|^2\gamma \log(1/\varepsilon_H(1-\gamma))}{(1-\gamma)^3}\|\pi_t' - \pi_{t-1}\|_{\infty, 1} }{(1-a)^t} \\ 
    &\leq \frac{2|A| \log(1/\min(\varepsilon_Q, \varepsilon_H) (1 - \gamma))}{(1-\gamma)^2}\cdot \frac{a + \eta\cdot\frac{2|A|\gamma }{(1-\gamma)} }{(1-a)^t} 
\end{align*}
To use Azuma's inequality we need to control the sum of the worst-case differences. To this end consider the following which holds for any $t$,
\begin{align*}
    \sum_{\tau=1}^{t} x_{\tau}^2 &\leq \sum_{\tau=1}^{t} \frac{4|A|^2 \log^2(1/\min(\varepsilon_Q, \varepsilon_H) (1 - \gamma))}{(1-\gamma)^4} \cdot \frac{\left(a + \eta\cdot\frac{2|A|\gamma }{(1-\gamma)}\right)^2 }{(1-a)^{2\tau}} \\
    &\leq \sum_{\tau=1}^{t}  \frac{4|A|^2 \log^2(1/\min(\varepsilon_Q, \varepsilon_H) (1 - \gamma))}{(1-\gamma)^4}\cdot \frac{2a^2 + \eta^2\cdot\frac{8|A|^2\gamma^2 }{(1-\gamma)^2}}{(1-a)^{2\tau}} \\
    &\leq \sum_{\tau=1}^{t}  \frac{4|A|^2 \log^2(1/\min(\varepsilon_Q, \varepsilon_H) (1 - \gamma))}{(1-\gamma)^4}\cdot \frac{2a^2 + \eta^2\cdot\frac{8|A|^2\gamma^2 }{(1-\gamma)^2}}{a(1-a)^{2t}}.
\end{align*}
A direct application of Azuma's inequality and a union bound leads to the following for any $t, \delta$ with probability at least $1 - \delta$ the following holds,
\[ |y_t| \leq |y_0|  + \frac{4|A| \log(1/\min(\varepsilon_Q, \varepsilon_H) (1 - \gamma))}{(1-\gamma)^2} \cdot \frac{\sqrt{(a + \frac{\eta^2}{a} \cdot \frac{4|A|^2\gamma^2 }{(1-\gamma)^2} )\log(2T/\delta)}}{(1-a)^{t}}  \]
Setting $a = \frac{2\eta |A|\gamma}{(1 - \gamma)}$, we get that for any $t, \delta$, with probability at least $\delta$ the following holds
    \[ |y_t| \leq |y_0|  + \frac{8|A|^{3/2} \sqrt{\gamma} \log(1/\min(\varepsilon_Q, \varepsilon_H) (1 - \gamma)) \sqrt{\log(2T/\delta)}}{(1-\gamma)^{5/2}} \cdot \frac{\sqrt{\eta}}{(1-a)^{t}}  \]
Replacing the definition of $y_t$ we get that for any $\delta$, with probability least $1 - \delta$
\begin{align*}
    |\epsilon_t| &\leq |\epsilon_0|(1-a)^t + \frac{8|A|^{3/2} \sqrt{\gamma} \log(1/\min(\varepsilon_Q, \varepsilon_H) (1 - \gamma)) \sqrt{\log(2T/\delta)}}{(1-\gamma)^{5/2}} \cdot \sqrt{\eta} \\
    &= \frac{8|A|^{3/2} \sqrt{\gamma} \log(1/\min(\varepsilon_Q, \varepsilon_H) (1 - \gamma)) \sqrt{\log(2T/\delta)}}{(1-\gamma)^{5/2}} \cdot \sqrt{\eta}.
\end{align*}

Then we have using Corollary~\ref{cor:qsamp} and that 
\[\bbE_{t-1}[\psi_t(\pi)] = \innerprod{\nabla V_{\mu}^{\pi_t}}{\pi}.\]
Further using Corollary~\ref{cor:hsamp} and the inputs to the H-sampler from Algorithm \ref{alg:cpi}, it follows that 
\[\bbE_{t-1}[\zeta_t(\pi)] = \bbE_{b_t}\left[\innerprod{\pi_{t} - \pi_{t-1}}{\nabla^2 V_{\mu}^{\bar{\pi}_t} \pi} \right] = \bbE_{b_t}\left[\innerprod{\nabla^2 V_{\mu}^{\bar{\pi}_t}(\pi_{t} - \pi_{t-1})}{ \pi} \right] = \innerprod{\nabla V_{\mu}^{\pi_t} - \nabla V_{\mu}^{\pi_{t-1}}}{\pi}.\]
We will now show that $\bbE[\innerprod{d_t}{\pi}]$. By definition we have that 





Using a union bound over all choices of $\pi$ and all timesteps $t \leq T$ we get that for any $\varepsilon, \delta$, with probability at least $1 - \delta$, we have that for any policy $\pi \in \Pi_{\varepsilon}$ and any time $t \leq T$,
\begin{equation}
    \label{eqn:tempeq}
    |\innerprod{d_t - \nabla V_{\mu}^{\pi_t}}{\pi}| \leq \frac{1}{(1-\gamma)^2}(1-a)^t + \frac{32 \sqrt{\gamma}|A|^{3/2}\log^{3/2}(12T^2|\Pi_{\epsilon}|/\delta)}{(1-\gamma)^{5/2}} \cdot \sqrt{\eta}.
\end{equation}

% We next show that the sequence $\{y_t\}$ is a martingale sequence over time $t$. To see this consider the following derivation, 
% \begin{align*}
%   \bbE_{t-1}[y_t] &= \frac{\bbE_{t-1}[\innerprod{\epsilon_t}{\pi}]}{(1-a)^t} =\frac{\bbE_{t-1}[\innerprod{(d_t - \nabla V_{\mu}^{\pi_t})}{\pi}]}{(1-a)^t} \\
%   &= \frac{1}{(1-a)^t} \left( (1-a) \bbE_{t-1}[\innerprod{(d_{t-1} - \nabla V_{\mu}^{\pi_{t-1}})}{\pi}] + a \left(\bbE_{t-1}[\psi_t(\pi)] - \innerprod{\nabla V_{\mu}^{\pi_t}}{\pi}\right) \right.\\
%   & \left. \qquad \qquad + (1-a) \left( \bbE_{t-1}[\zeta_t(\pi)] - \innerprod{(\nabla V_{\mu}^{\pi_t} - \nabla V_{\mu}^{\pi_{t-1}})}{\pi} \right) \right) \\
%   &= \frac{(1-a)\innerprod{\epsilon_{t-1}}{\pi}}{(1-a)^t} = y_{t-1}  
% \end{align*}
We now wish to use Azuma's inequality to show concentration for the martingale sequence. 
Furthermore, note that for any policies $\pi, \pi'$ Lemma \ref{lem:grad} implies that $\innerprod{\nabla V_{\mu}^{\pi}}{\pi'} \leq \frac{1}{(1-\gamma)^2}$. Using the above derivations and Lemma \ref{lem:smooth}, we can now bound the differences of the martingale sequences as follows which holds for all $t, \delta$ with probability at least $1 - \delta$ via a union bound, 





For the rest of the argument we will generate a crude bound over $\|d_t\|_{1, \infty}$. To this end will bound $\innerprod{d_t}{\pi}$ for all $\pi \in \B_{\infty, 1}$. By Lemma \ref{lem:dualnorm} since $\|\cdot\|_{\infty,1}$ and $\|\cdot\|_{1, \infty}$ are duals of each other we get the required bound. Therefore consider any $\pi \in \B_{\infty, 1}$. Using the definition of $d_t$ and defining $\phi_t$ and $\zeta_t$ analogously as before we get that 
\na{We should condition out the events before itself}
\begin{align*}
    \innerprod{d_t}{\pi} &\leq (1-a)\innerprod{d_{t-1}}{\pi} + a |\phi_t| + (1-a)\zeta_t \\
    &\leq (1-a)\innerprod{d_{t-1}}{\pi} + a \frac{1}{(1-\gamma)^2} + \eta \\
\end{align*}
Now we will show by induction that $\policynorm{d_t}^* \leq 5/4$. For the base case note that $\policynorm{d_t}^* = \policynorm{\nabla f(\pi_0, \xi_0)}^* \leq 1$. For the inductive case, it follows via the following computation using the choice of $a$,
\begin{align*}
    \policynorm{d_t}^* 
    &\leq (1-a)\policynorm{d_{t-1}}^* + a + \eta \\
    &\leq (1-a)5/4 + 5a/4 \leq 5/4.\\
\end{align*}
This in particular implies that for all $t$, $\policynorm{d_t - \nabla F(\pi_t)}^* \leq 9/4$. Now consider any $\pi \in \Pi$, by the covering property we have that there exists a $\pi' \in \Pi_{\varepsilon}$ such that for all $t$, 
\[|\innerprod{d_t - \nabla F(\pi_t)}{\pi}| \leq |\innerprod{d_t - \nabla F(\pi_t)}{\pi'}| + 9/4 \varepsilon.\] 
Combining the above with \eqref{eqn:tempeq} completes the proof. 
% Consider the definition of the variance as required in Friedman's inequality 

% \[ \sigma_t^2 \defeq \sum_{j=0}^{t - 1}\bbE_{j}[X_t^2]\]

% It is now easy to see that
% \begin{align*}
%     \sigma_t^2 &= \sum_{j=0}^{t - 1} \frac{a^2\sigma^2 + (1-a)^2\eta^2\left(\innerprod{d_t}{H_1v - H_2v}\right)^2}{(1-a)^{2t}}
% \end{align*}

% At this point we need the inf-inf boundedness of $H$ to say that $H_1v - H_2v$ is bounded in inf-norm if that is the case we can replace it with a $v'$ and get that 

% \begin{align*}
%     \sigma_t^2 &\leq \sum_{j=0}^{t - 1} \frac{a^2\sigma^2 + 2(1-a)^2\eta^2L^2 \left(\innerprod{\nabla F(x_t)}{v'}\right)^2 +  2(1-a)^2\eta^2L^2 \left(\innerprod{\epsilon_{t-1}}{v'}\right)^2}{(1-a)^{2t}} \\
%     &\leq \sum_{j=0}^{t - 1} \frac{a^2\sigma^2 + 2(1-a)^2\eta^2L^2 G^2 +  2(1-a)^2\eta^2L^2 \left(\innerprod{\epsilon_{t-1}}{v'}\right)^2}{(1-a)^{2t}} \\
%     &= \sum_{j=0}^{t - 1} \frac{a^2\sigma^2 + 2(1-a)^2\eta^2L^2 G^2}{(1-a)^{2t}} + \sum_{j=0}^{t - 1} \frac{2(1-a)^2\eta^2L^2 \left(\innerprod{\epsilon_{t-1}}{v'}\right)^2}{(1-a)^{2t}} \\
%     &= \frac{a^2\sigma^2 + 2(1-a)^2\eta^2L^2 G^2}{a(1-a)} \cdot \frac{1}{(1-a)^{2t}} + \sum_{j=0}^{t - 1} \frac{2(1-a)^2\eta^2L^2 \left(\innerprod{\epsilon_{t-1}}{v'}\right)^2}{(1-a)^{2t}} \\
%     &= \frac{c_1}{(1-a)^{2t}} + \sum_{j=0}^{t - 1} \frac{c_2 \left(\innerprod{\epsilon_{t-1}}{v'}\right)^2}{(1-a)^{2t}}
% \end{align*}





% The inductive hypothesis will be eventually to have some bound $\Gamma_t$ for the inner product with every vector $v'$ with probability $1/(\delta T)$ so we will have something like (ignoring the constant term)

% \begin{align*}
%     \Gamma_t \sim (1-a)^{t}\sigma_t \log\left(\frac{\|\Pi\|T}{d}\right)
%     \leq \sqrt{c_1^2 + \sum_{j=0}^{t - 1} c_2 \left(\innerprod{\epsilon_{t-1}}{v'}\right)^2(1-a)^{2(t-1-j)}}
% \end{align*}

% Suppose we even assume some constant behavior for $\Gamma$s we will get something like

% \begin{align*}
%     \Gamma_t \leq \sqrt{c_1^2 +  \frac{c_2}{a} \Gamma} \cdot \log\left(\frac{\|\Pi\|T}{d}\right)
% \end{align*}

% Lets approximate these terms $c_1^2 ~ \eta$. $c_2/a \sim \eta$ as well. Therefore we are getting 

% \[\Gamma_t \leq \sqrt{\eta + \eta*\Gamma} \cdot \log()\]


% This should maintain $\Gamma \leq 2\sqrt{\eta} \cdot \log $ as long as 
% $ 2\eta^{3/2}\log \leq \eta \Leftarrow \eta \leq \frac{1}{4 \log^2}$
\end{proof}

